When RL Meets Adaptive Speculative Training: A Unified Training-Serving System

Speculative decoding can significantly accelerate LLM serving, yet most deployments today disentangle speculator training from serving, treating speculator training as a standalone offline modeling problem. We show that this decoupled formulation introduces substantial deployment and adaptation lag: (1) high time-to-serve, since a speculator must be trained offline for a considerable period before deployment; (2) delayed utility feedback, since the true end-to-end decoding speedup is only known after training and cannot be inferred reliably from acceptance rate alone due to model-architecture and system-level overheads; and (3) domain-drift degradation, as the target model is repurposed to new domains and the speculator becomes stale and less effective. To address these issues, we present Aurora, a unified training-serving system that closes the loop by continuously learning a speculator directly from live inference traces. Aurora reframes online speculator learning as an asynchronous reinforcement-learning problem: accepted tokens provide positive feedback, while rejected speculator proposals provide implicit negative feedback that we exploit to improve sample efficiency. Our design integrates an SGLang-based inference server with an asynchronous training server, enabling hot-swapped speculator updates without service interruption. Crucially, Aurora supports day-0 deployment: a speculator can be served immediately and rapidly adapted to live traffic, improving system performance while providing immediate utility feedback. Across experiments, Aurora achieves a 1.5x day-0 speedup on recently released frontier models (e.g., MiniMax M2.1 229B and Qwen3-Coder-Next 80B). Aurora also adapts effectively to distribution shifts in user traffic, delivering an additional 1.25x speedup over a well-trained but static speculator on widely used models (e.g., Qwen3 and Llama3).

==> sections/figureA1.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{../fig/slime-rl-design.png}
    \caption{Left}
    \label{fig:left_wide}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/main-results.png}
    \caption{Right}
    \label{fig:right_wide}
  \end{subfigure}
  \caption{We build a good spec online system, we study advanced speculative decoding and found that there is marginal benefit when using tree attention (\cite{...} and ...)}
  \label{fig:two_col_two_subfigs}
\end{figure*}
\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{../fig/slime-rl-design.png}
    \caption{Left}
    \label{fig:left_wide}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/tree_attn.pdf}
    \caption{Right}
    \label{fig:right_wide}
  \end{subfigure}
  \caption{Two-column wide figure with two subfigures.}
  \label{fig:two_col_two_subfigs}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{../fig/diagram.pdf}
    \label{fig:system_diagram}
    \caption{The unified training-serving system. During inference, the target model serves requests while a draft speculator generates proposals. As the system runs, interaction traces (prompts, accepted tokens, and verification signals) are streamed into a data buffer. A separate training server continuously samples from this buffer to perform small, frequent gradient updates on the speculator, enabling rapid adaptation to the current workload without interrupting the main inference pipeline. Updated speculator weights are asynchronously pushed back to the inference server, closing the loop and improving future decoding efficiency under non-stationary request distributions. The two curves at the bottom illustrate: training progress drives a rising acceptance-length curve, and async weight pushes translate that into monotonic throughput gains at inference.}
\end{figure*}



==> sections/intro_old.tex <==
Speculative decoding~\cite{leviathan2023fast,chen2023accelerating} has emerged as an effective solution to accelerate LLM inference. The key idea is to employ a lightweight \emph{draft model} to rapidly generate candidate token sequences, which are then verified in parallel by the larger \emph{target model}. Since the target model can evaluate multiple positions simultaneously during verification, multiple tokens can be accepted in a single forward pass when the draft model's predictions align with what the target model would have produced. 

This approach maintains the exact output distribution of the target model while significantly reducing inference latency.

The efficacy of speculative decoding hinges critically on the draft model's ability to accurately predict the target model's outputs, measured by the \emph{token acceptance rate} $\alpha$. When draft tokens frequently match the target model's preferences, fewer verification rounds are needed, leading to greater speedups. Conversely, when the draft model's predictions diverge from the target, speculation failures accumulate and the benefits diminish.

\paragraph{EAGLE and Feature-Level Speculation.}
Methods like EAGLE~\cite{li2024eagle} advance speculative decoding by operating at the feature level rather than the token level. Instead of training an independent draft model, EAGLE reuses the top-layer features from the target model (the representations immediately before the language modeling head) and trains a lightweight draft head to autoregressively predict the next feature. This approach leverages the rich information already computed by the target model, achieving significantly better acceptance rates compared to vanilla speculative sampling with independent draft models.

EAGLE-3~\cite{li2025eagle3} further improves upon this design with two key innovations: (1) removing the feature prediction constraint in favor of direct token prediction through a technique called \emph{training-time test}, and (2) replacing reliance on top-layer features with multi-layer feature fusion that integrates low-, mid-, and high-level representations from the target model. These improvements enable EAGLE-3 to achieve speedups of 4-6$\times$ over vanilla autoregressive decoding, with average acceptance lengths exceeding 6 tokens per verification cycle.

\paragraph{The Distribution Shift Problem.}
Despite these advances, a fundamental limitation persists: draft models remain static after deployment. They are trained on fixed datasets that may not reflect the actual distribution of queries encountered during inference~\cite{liu2024online}. This distribution shift manifests in several ways:
\begin{itemize}
    \item \textbf{Domain mismatch}: A draft model trained on general conversational data may struggle with specialized domains such as code generation or mathematical reasoning.
    \item \textbf{User-specific patterns}: Individual users or applications exhibit consistent linguistic patterns that differ from training data distributions.
    \item \textbf{Temporal drift}: Language usage and topics evolve over time, and static models cannot adapt to emerging terminology or conventions.
\end{itemize}

When distribution shift occurs, the draft model's predictions increasingly diverge from the target model's outputs, leading to more speculation failures and reduced speedups. In extreme cases, a poorly matched draft model provides minimal benefit over standard autoregressive decoding.

\paragraph{Online Speculative Decoding.}
Liu et al.~\cite{liu2024online} introduced online speculative decoding (OSD) to address distribution shift by continuously updating the draft model during deployment. The key insight is that speculative decoding naturally produces supervision signals: when draft tokens are rejected, both the draft model's incorrect prediction and the target model's correct output are observed. These \emph{discarded tokens} represent precisely the cases where the draft model needs improvement. By applying knowledge distillation on the fly, OSD adapts the draft model to the actual query distribution, improving token acceptance rates by 10-65\% on diverse datasets.

\paragraph{Challenges for EAGLE3 Online Training.}
While OSD demonstrates the potential of online adaptation, applying it to EAGLE3-style draft models presents unique challenges:

\textbf{(1) Memory overhead}: EAGLE3 draft models require access to target model hidden states during both inference and training. Running the target model twice---once for serving and once for computing training gradients---would double GPU memory requirements.

\textbf{(2) Training efficiency}: Speculative decoding produces multiple rejection branches per verification cycle. Each branch contains tokens that were predicted by the draft but rejected by the target. Processing each branch independently wastes computation.

\textbf{(3) Architecture alignment}: EAGLE3's training-time test technique unrolls the draft model for multiple steps during training. Online training must maintain this structure while adapting to streaming data.

==> sections/method_old.tex <==
% \section{Method}
\label{sec:method}


\section{Online Speculator Training Framework}
\section{Datasets}
\label{sec:dataset}

We conduct our inference-time training experiments on a diverse multi-domain dataset consisting of 44,473 user queries spanning five distinct domains. The dataset is designed to evaluate test-time adaptation across varied reasoning and generation tasks representative of real-world language model deployment scenarios.

\subsection{Dataset Composition}

The training corpus comprises samples from five domains, as detailed in Table~\ref{tab:dataset_composition}:

\begin{table}[h]
\centering
\caption{Multi-domain dataset composition for inference-time training experiments.}
\label{tab:dataset_composition}
\begin{tabular}{lrr}
\toprule
\textbf{Domain} & \textbf{Samples}  \\
\midrule
Code Generation & 10,000\\
Finance & 10,000\\
Conversational Instructions (CIP) & 10,000\\
Mathematical Reasoning (GSM8K) & 7,473\\
Text-to-SQL (Spider) & 7,000 \\
\midrule
\textbf{Total} & \textbf{44,473} \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Code Generation} (10,000 samples, 22.5\%) comprises programming tasks requiring code synthesis from natural language specifications, testing the model's ability to generate syntactically correct and functionally appropriate code.

\paragraph{Finance} (10,000 samples, 22.5\%) includes financial reasoning queries covering portfolio management, investment strategies, and economic analysis, requiring domain-specific knowledge and numerical reasoning.

\paragraph{Conversational Instructions (CIP)} (10,000 samples, 22.5\%) consists of general instruction-following tasks covering everyday problem-solving scenarios, from household repairs to general advice.

\paragraph{Mathematical Reasoning (GSM8K)} (7,473 samples, 16.8\%) contains grade school math word problems requiring multi-step arithmetic reasoning~\citep{cobbe2021training}.

\paragraph{Text-to-SQL (Spider)} (7,000 samples, 15.7\%) comprises natural language to SQL translation tasks requiring database schema understanding and structured query generation~\citep{yu2018spider}.

\subsection{Data Format and Processing}

Each sample consists of a single user query in conversational format without ground-truth assistant responses, reflecting realistic inference-time scenarios where the model must generate responses autonomously. This design enables our method to learn from the model's own speculative decoding process during inference, creating a self-supervised training signal from accepted and rejected draft tokens produced by the EAGLE-3 speculative decoding algorithm.

We use two versions of the dataset: (1) \textit{mixed-data} with source-ordered samples grouped by domain, and (2) \textit{ordered-data} with randomly shuffled samples across domains to prevent domain-specific overfitting during streaming updates. All experiments reported in this work use the shuffled version to ensure domain-balanced online learning. Each sample is formatted as a JSON object with an identifier indicating its source domain and a conversations list containing the user query.

The multi-domain composition ensures our inference-time training method must continuously adapt to heterogeneous task distributions, testing the robustness of the learning signal derived from speculative decoding dynamics across diverse reasoning patterns. This design choice reflects realistic deployment scenarios where production language models encounter rapid shifts in task distribution and must adapt without explicit supervision.


\section{Training Strategy}
\label{sec:training_strategy}
\begin{table}[t]
\centering
\caption{Training configurations compared in our experiments. All use Qwen3-8B (target) and EAGLE-3-Qwen3-8B (draft) with learning rate $10^{-6}$, processing 44.5K multi-domain prompts streamed as inference traffic.}
\label{tab:experiment_configs}
\small
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
\textbf{Configuration} & \textbf{Train} & \textbf{Accept} & \textbf{Tree} & \textbf{NTP} \\
\midrule
Baseline & \xmark & -- & -- & -- \\
Normal-Fine & \cmark & \cmark & \xmark & \xmark \\
Normal-Fine+NTP & \cmark & \cmark & \xmark & \cmark \\
Tree & \cmark & \cmark & \cmark & \xmark \\
Tree+NTP & \cmark & \cmark & \cmark & \cmark \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize
\item Train: online gradient updates enabled; Accept: learn from accepted tokens; Tree: tree attention on discarded branches (top-$k$=10); NTP: next-token prediction loss on accepted tokens.
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{table}[t]
\centering
\caption{Shared hyperparameters across all training configurations. Constant LR maintains plasticity for online learning.}
\label{tab:hyperparameters}
\small
\begin{tabular}{lr}
\toprule
\textbf{Parameter} & \textbf{Value} \\
\midrule
\multicolumn{2}{l}{\textit{Training}} \\
Learning Rate & $10^{-6}$ (constant) \\
Warmup Steps & 400 \\
Global Batch Size & 32 \\
Draft/Target Micro-batch & 1 / 4 \\
Optimizer & AdamW \\
Weight Decay & 0.0 \\
Gradient Clipping & 0.5 \\
Precision & BF16 + FP32 \\
\midrule
\multicolumn{2}{l}{\textit{Speculative Decoding}} \\
Speculative Steps & 7 \\
Draft Tokens per Step & 8 \\
Top-$k$ Sampling & 1 \\
Tree Attention & \cmark \\
\midrule
\multicolumn{2}{l}{\textit{Sequence \& Loss}} \\
Max Sequence Length & 2,048 \\
TTT Length & 5 \\
Loss Weights ($\lambda$) & 1.0 (all) \\
Top-$k$ Filter (discard) & 10 \\
Divergence & Reverse KL \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[b]
\centering
\caption{Training configurations compared in our experiments. All settings use Qwen3-8B as the target model and EAGLE-3-Qwen3-8B as the draft model with learning rate $10^{-6}$.}
\label{tab:experiment_configs}
\small
\begin{threeparttable}
\begin{tabular}{lccc}
\toprule
\textbf{Config} & \textbf{Accept} & \textbf{Discard} & \textbf{NTP} \\
\midrule
Baseline      & \xmark & \xmark & \xmark \\
Normal        & \cmark & \xmark & \xmark \\
Normal+NTP    & \cmark & \xmark & \cmark \\
Discard+NTP   & \cmark & \cmark & \cmark \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\small
\item Accept: train on accepted tokens; Discard: train on rejected tokens (top-$k$=10); NTP: next-token prediction loss.
\end{tablenotes}
\end{threeparttable}
\end{table}
We evaluate our inference-time training approach across multiple training configurations to isolate the contributions of different learning signals available during speculative decoding. Our experimental design compares static baselines against online learning methods that leverage accepted tokens, discarded tokens, or both.

\subsection{Model Architecture}

We employ EAGLE-3~\citep{li2024eagle2} as our speculative decoding framework, which uses a lightweight draft model to propose candidate token sequences that are subsequently verified by the target model in parallel. Specifically:

\paragraph{Target Model:} Qwen3-8B~\citep{qwen3}, an 8-billion parameter instruction-tuned language model serving as the authoritative generation model.

\paragraph{Draft Model:} EAGLE-3-Qwen3-8B, a specialized speculative draft model initialized from a pretrained checkpoint. The draft model is significantly smaller in computational cost per token while sharing the same vocabulary as the target model, enabling efficient parallel verification.

\paragraph{Speculative Configuration:} We use 7 speculative steps with top-1 sampling and 8 draft tokens per speculation step, producing speculative trees that balance acceptance rate and speculation overhead.

\subsection{Training Configurations}

To understand the value of different supervision signals during inference-time training, we compare four training modes:

\subsubsection{Baseline (No Training)}

The baseline configuration serves inference requests using a static pretrained draft model without any online adaptation. This represents standard speculative decoding deployment where the draft model parameters remain frozen. The baseline provides a reference point for measuring the benefits of inference-time learning.

\subsubsection{Normal Training}

Normal training performs online gradient updates on the draft model using only accepted tokens—those that match the target model's output during verification. This approach corresponds to standard on-policy imitation learning, where the draft model learns to mimic the target model's distribution on tokens that were successfully predicted. The training signal is sparse, as only a subset of proposed tokens are accepted.

\subsubsection{Discard Training}

Discard training leverages the rejected tokens during speculative verification, which provide dense supervision about where the draft model's distribution diverges from the target model. We apply tree attention~\citep{miao2023specinfer} to efficiently process the speculative tree structure and compute losses over discarded branches. To stabilize learning from negative examples, we apply top-$k$ filtering with $k=10$ to focus on high-confidence disagreements and weight the discarded loss term with $\lambda_{\text{discard}}=1.0$.

\subsubsection{Discard + NTP Training}

To combine complementary supervision signals, we augment discard training with a next-token prediction (NTP) loss computed on accepted tokens. This configuration learns from both positive examples (accepted tokens) and negative examples (discarded tokens), weighted by $\lambda_{\text{NTP}}=1.0$. The combined objective encourages the draft model to both match the target's distribution on successful predictions and avoid divergence patterns revealed by rejected tokens.

\subsection{Optimization and Hyperparameters}

All online training configurations share a common optimization setup designed for stable streaming updates under inference workload constraints:

\paragraph{Optimizer:} AdamW with weight decay $\beta=0.0$ and gradient clipping at max norm 0.5.

\paragraph{Learning Rate:} We use a constant learning rate of $\eta=1\times10^{-6}$ after a brief linear warmup over 400 steps (0.05\% of total training). This constant schedule is critical for test-time training scenarios where the model must maintain plasticity for continuous adaptation without forgetting~\citep{sun2020test}.

\paragraph{Batch Configuration:} Global batch size of 32 for draft model training, with micro-batch sizes of 1 for draft model forward passes and 4 for target model verification. These asymmetric batch sizes balance training stability with inference throughput requirements.

\paragraph{Context Window:} Maximum sequence length of 2,048 tokens with a test-time training (TTT) length of 5 tokens, defining the local context window for each gradient update.

\paragraph{Mixed Precision:} BF16 computation with FP32 master weights and gradients cast to FP32 before optimization, following best practices for training stability~\citep{micikevicius2018mixed}.

\paragraph{Loss Function:} Reverse KL divergence $D_{\text{KL}}(p_{\text{target}} \| p_{\text{draft}})$ to encourage the draft model to cover the target model's distribution, minimizing false rejections during speculative verification.

\subsection{Infrastructure and Efficiency}

To enable online training without degrading inference throughput, we employ a split-GPU architecture with RPC-based data transfer:

\paragraph{GPU Allocation:} The target model runs inference on GPU 0 while the draft model trains on GPU 1, eliminating resource contention between serving and learning.

\paragraph{Data Transfer:} Hidden states and verification outcomes are transmitted via RPC from the inference server to the training process, with storage buffers co-located on GPU 1 to avoid redundant memory copies.

\paragraph{Asynchronous Updates:} Gradient updates proceed asynchronously with respect to inference, ensuring that serving latency remains unaffected by training overhead.

This infrastructure design achieves online learning with minimal impact on user-facing metrics, making inference-time training practical for production deployment.

\subsection{Experimental Design}

We run controlled experiments comparing all four training configurations (Baseline, Normal, Discard, Discard+NTP) in parallel across separate GPU pairs using identical workloads sampled from the shuffled multi-domain dataset (Section~\ref{sec:dataset}). Each experiment processes up to 2 million inference requests, with draft model checkpoints saved every 5,000 training steps and metrics logged every 10 steps. This design isolates the effect of training strategy while controlling for dataset distribution, hardware variability, and inference workload characteristics.


